DYNAFED: Tackling Client Data Heterogeneity with Global Dynamics

The Federated Learning (FL) paradigm is known to face challenges under heterogeneous client data. Local training on non-iid distributed data results in deflected local optimum, which causes the client models drift further away from each other and degrades the aggregated global model's performance. A natural solution is to gather all client data onto the server, such that the server has a global view of the entire data distribution. Unfortunately, this reduces to regular training, which compromises clients' privacy and conflicts with the purpose of FL. In this paper, we put forth an idea to collect and leverage global knowledge on the server without hindering data privacy. We unearth such knowledge from the dynamics of the global model's trajectory. Specifically, we first reserve a short trajectory of global model snapshots on the server. Then, we synthesize a small pseudo dataset such that the model trained on it mimics the dynamics of the reserved global model trajectory. Afterward, the synthesized data is used to help aggregate the deflected clients into the global model. We name our method Dynafed, which enjoys the following advantages: 1) we do not rely on any external on-server dataset, which requires no additional cost for data collection; 2) the pseudo data can be synthesized in early communication rounds, which enables Dynafed to take effect early for boosting the convergence and stabilizing training; 3) the pseudo data only needs to be synthesized once and can be directly utilized on the server to help aggregation in subsequent rounds. Experiments across extensive benchmarks are conducted to showcase the effectiveness of Dynafed. We also provide insights and understanding of the underlying mechanism of our method.

==> cvpr2023-author_kit-v1_1-1/latex/bib2.tex <==
@string(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@string(IJCV = {Int. J. Comput. Vis.})
@string(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@string(ICCV= {Int. Conf. Comput. Vis.})
@string(ECCV= {Eur. Conf. Comput. Vis.})
@string(NIPS= {Adv. Neural Inform. Process. Syst.})
@string(ICPR = {Int. Conf. Pattern Recog.})
@string(BMVC= {Brit. Mach. Vis. Conf.})
@string(TOG= {ACM Trans. Graph.})
@string(TIP  = {IEEE Trans. Image Process.})
@string(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@string(TMM  = {IEEE Trans. Multimedia})
@string(ACMMM= {ACM Int. Conf. Multimedia})
@string(ICME = {Int. Conf. Multimedia and Expo})
@string(ICASSP=	{ICASSP})
@string(ICIP = {IEEE Int. Conf. Image Process.})
@string(ACCV  = {ACCV})
@string(ICLR = {Int. Conf. Learn. Represent.})
@string(IJCAI = {IJCAI})
@string(PR   = {Pattern Recognition})
@string(AAAI = {AAAI})
@string(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@string(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})
@string(SPL	= {IEEE Sign. Process. Letters})
@string(VR   = {Vis. Res.})
@string(JOV	 = {J. Vis.})
@string(TVC  = {The Vis. Comput.})
@string(JCST  = {J. Comput. Sci. Tech.})
@string(CGF  = {Comput. Graph. Forum})
@string(CVM = {Computational Visual Media})
@string(PAMI  = {IEEE TPAMI})
@string(IJCV  = {IJCV})
@string(CVPR  = {CVPR})
@string(ICCV  = {ICCV})
@string(ECCV  = {ECCV})
@string(NIPS  = {NeurIPS})
@string(ICPR  = {ICPR})
@string(BMVC  =	{BMVC})
@string(TOG   = {ACM TOG})
@string(TIP   = {IEEE TIP})
@string(TVCG  = {IEEE TVCG})
@string(TCSVT = {IEEE TCSVT})
@string(TMM   =	{IEEE TMM})
@string(ACMMM = {ACM MM})
@string(ICME  =	{ICME})
@string(ICASSP=	{ICASSP})
@string(ICIP  = {ICIP})
@string(ACCV  = {ACCV})
@string(ICLR  = {ICLR})
@string(IJCAI = {IJCAI})
@string(PR = {PR})
@string(AAAI = {AAAI})
@string(CVPRW= {CVPRW})
@string(CSVT = {IEEE TCSVT})
@article{hu2021analysis,
	title        = {Analysis of biased stochastic gradient descent using sequential semidefinite programs},
	author       = {Hu, Bin and Seiler, Peter and Lessard, Laurent},
	year         = 2021,
	journal      = {Mathematical Programming},
	publisher    = {Springer},
	volume       = 187,
	number       = 1,
	pages        = {383--408}
}
@article{jacot2018neural,
	title        = {Neural tangent kernel: Convergence and generalization in neural networks},
	author       = {Jacot, Arthur and Gabriel, Franck and Hongler, Cl{\'e}ment},
	year         = 2018,
	journal      = {Advances in neural information processing systems},
	volume       = 31
}
@book{wolfgang1998ordinary,
	title        = {Ordinary differential equations},
	author       = {Wolfgang, Walter and Walter, Wolfgang and Walter, Wolfgang Ludwig},
	year         = 1998,
	publisher    = {Springer Science \& Business Media},
	volume       = 182
}
@misc{Authors14,
	title        = {The frobnicatable foo filter},
	author       = {FirstName LastName},
	year         = 2014,
	note         = {Face and Gesture submission ID 324. Supplied as supplemental material {\tt fg324.pdf}}
}
@misc{Authors14b,
	title        = {Frobnication tutorial},
	author       = {FirstName LastName},
	year         = 2014,
	note         = {Supplied as supplemental material {\tt tr.pdf}}
}
@article{Alpher02,
	title        = {Frobnication},
	author       = {FirstName Alpher},
	year         = 2002,
	journal      = PAMI,
	volume       = 12,
	number       = 1,
	pages        = {234--778}
}
@article{Alpher03,
	title        = {Frobnication revisited},
	author       = {FirstName Alpher and  FirstName Fotheringham-Smythe},
	year         = 2003,
	journal      = {Journal of Foo},
	volume       = 13,
	number       = 1,
	pages        = {234--778}
}
@article{Alpher04,
	title        = {Can a machine frobnicate?},
	author       = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
	year         = 2004,
	journal      = {Journal of Foo},
	volume       = 14,
	number       = 1,
	pages        = {234--778}
}
@inproceedings{Alpher05,
	title        = {Can a computer frobnicate?},
	author       = {FirstName Alpher and FirstName Gamow},
	year         = 2005,
	booktitle    = CVPR,
	pages        = {234--778}
}
%%%% Fed background
@article{zhou2021efficient,
	title        = {Efficient neural network training via forward and backward propagation sparsification},
	author       = {Zhou, Xiao and Zhang, Weizhong and Chen, Zonghao and Diao, Shizhe and Zhang, Tong},
	year         = 2021,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 34,
	pages        = {15216--15229}
}
@inproceedings{xie2020zeno++,
	title        = {Zeno++: Robust fully asynchronous SGD},
	author       = {Xie, Cong and Koyejo, Sanmi and Gupta, Indranil},
	year         = 2020,
	booktitle    = {International Conference on Machine Learning},
	pages        = {10495--10503},
	organization = {PMLR}
}
@inproceedings{xie2019zeno,
	title        = {Zeno: Distributed stochastic gradient descent with suspicion-based fault-tolerance},
	author       = {Xie, Cong and Koyejo, Sanmi and Gupta, Indranil},
	year         = 2019,
	booktitle    = {International Conference on Machine Learning},
	pages        = {6893--6901},
	organization = {PMLR}
}
@book{wainwright2019high,
	title        = {High-dimensional statistics: A non-asymptotic viewpoint},
	author       = {Wainwright, Martin J},
	year         = 2019,
	publisher    = {Cambridge University Press},
	volume       = 48
}
@article{polyak1964gradient,
	title        = {Gradient methods for solving equations and inequalities},
	author       = {Polyak, Boris T},
	year         = 1964,
	journal      = {USSR Computational Mathematics and Mathematical Physics},
	publisher    = {Elsevier},
	volume       = 4,
	number       = 6,
	pages        = {17--32}
}
@article{kuditipudi2019explaining,
	title        = {Explaining landscape connectivity of low-cost solutions for multilayer nets},
	author       = {Kuditipudi, Rohith and Wang, Xiang and Lee, Holden and Zhang, Yi and Li, Zhiyuan and Hu, Wei and Ge, Rong and Arora, Sanjeev},
	year         = 2019,
	journal      = {Advances in neural information processing systems},
	volume       = 32
}
@inproceedings{stich2018local,
	title        = {Local SGD Converges Fast and Communicates Little},
	author       = {Stich, Sebastian U},
	year         = 2018,
	booktitle    = {International Conference on Learning Representations}
}
@inproceedings{li2020convergence,
	title        = {On the Convergence of FedAvg on Non-IID Data},
	author       = {Li, Xiang and Huang, Kaixuan and Yang, Wenhao and Wang, Shusen and Zhang, Zhihua},
	year         = 2020,
	booktitle    = {International Conference on Learning Representations}
}
@article{hoffman2018algorithms,
	title        = {Algorithms and theory for multiple-source adaptation},
	author       = {Hoffman, Judy and Mohri, Mehryar and Zhang, Ningshan},
	year         = 2018,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 31
}
@article{konevcny2016federated,
	title        = {Federated learning: Strategies for improving communication efficiency},
	author       = {Kone{\v{c}}n{\`y}, Jakub and McMahan, H Brendan and Yu, Felix X and Richt{\'a}rik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
	year         = 2016,
	journal      = {arXiv preprint arXiv:1610.05492}
}
@article{yang2019federated,
	title        = {Federated machine learning: Concept and applications},
	author       = {Yang, Qiang and Liu, Yang and Chen, Tianjian and Tong, Yongxin},
	year         = 2019,
	journal      = {ACM Transactions on Intelligent Systems and Technology (TIST)},
	publisher    = {ACM New York, NY, USA},
	volume       = 10,
	number       = 2,
	pages        = {1--19}
}
%noniid
@article{hsu2019measuring,
	title        = {Measuring the effects of non-identical data distribution for federated visual classification},
	author       = {Hsu, Tzu-Ming Harry and Qi, Hang and Brown, Matthew},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1909.06335}
}
%fedavg convergence
@inproceedings{mcmahan2017communication,
	title        = {Communication-efficient learning of deep networks from decentralized data},
	author       = {McMahan, H Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and others},
	year         = 2017,
	booktitle    = {AISTATS}
}
@article{sahu2018convergence,
	title        = {On the convergence of federated optimization in heterogeneous networks},
	author       = {Sahu, Anit Kumar and Li, Tian and Sanjabi, Maziar and Zaheer, Manzil and Talwalkar, Ameet and Smith, Virginia},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1812.06127}
}
@inproceedings{zinkevich2010parallelized,
	title        = {Parallelized stochastic gradient descent},
	author       = {Zinkevich, Martin and Weimer, Markus and Li, Lihong and Smola, Alex J},
	year         = 2010,
	booktitle    = {NIPS}
}
@article{zhou2017convergence,
	title        = {On the convergence properties of a $ K $-step averaging stochastic gradient descent algorithm for nonconvex optimization},
	author       = {Zhou, Fan and Cong, Guojing},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1708.01012}
}
%drift
@article{zhao2018federated,
	title        = {Federated learning with non-iid data},
	author       = {Zhao, Yue and Li, Meng and Lai, Liangzhen and Suda, Naveen and Civin, Damon and Chandra, Vikas},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1806.00582}
}
@inproceedings{karimireddy2019scaffold,
	title        = {SCAFFOLD: Stochastic controlled averaging for on-device federated learning},
	author       = {Karimireddy, Sai Praneeth and Kale, Satyen and Mohri, Mehryar and Reddi, Sashank J and Stich, Sebastian U and Suresh, Ananda Theertha},
	year         = 2020,
	booktitle    = {ICML}
}
@inproceedings{Acar2021Dyn,
	title        = {Federated Learning Based on Dynamic Regularization},
	author       = {Durmus Alp Emre Acar and Yue Zhao and Ramon Matas Navarro and Matthew Mattina and Paul N. Whatmough and Venkatesh Saligrama},
	year         = 2021,
	booktitle    = {ICLR},
	timestamp    = {Thu, 14 Oct 2021 10:00:36 +0200},
	biburl       = {https://dblp.org/rec/conf/iclr/AcarZNMWS21.bib},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
%fedprox
@inproceedings{li2020federated,
	title        = {Federated optimization in heterogeneous networks},
	author       = {Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
	year         = 2020,
	booktitle    = {MLSys}
}
@inproceedings{li2019feddane,
	title        = {Feddane: A federated newton-type method},
	author       = {Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smithy, Virginia},
	year         = 2019,
	booktitle    = {2019 53rd Asilomar Conference on Signals, Systems, and Computers},
	pages        = {1227--1231},
	organization = {IEEE}
}
@article{yao2019federated,
	title        = {Federated Learning with Unbiased Gradient Aggregation and Controllable Meta Updating},
	author       = {Yao, Xin and Huang, Tianchi and Zhang, Rui-Xiao and Li, Ruiyu and Sun, Lifeng},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1910.08234}
}
@inproceedings{li2021model,
	title        = {Model-contrastive federated learning},
	author       = {Li, Qinbin and He, Bingsheng and Song, Dawn},
	year         = 2021,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {10713--10722}
}
%model connectivity
@article{garipov2018loss,
	title        = {Loss surfaces, mode connectivity, and fast ensembling of dnns},
	author       = {Garipov, Timur and Izmailov, Pavel and Podoprikhin, Dmitrii and Vetrov, Dmitry P and Wilson, Andrew G},
	year         = 2018,
	journal      = {Advances in neural information processing systems},
	volume       = 31
}
@inproceedings{draxler2018essentially,
	title        = {Essentially no barriers in neural network energy landscape},
	author       = {Draxler, Felix and Veschgini, Kambis and Salmhofer, Manfred and Hamprecht, Fred},
	year         = 2018,
	booktitle    = {International conference on machine learning},
	pages        = {1309--1318},
	organization = {PMLR}
}
%server agg
% good perform fedavg
@inproceedings{li2022federated,
	title        = {Federated learning on non-iid data silos: An experimental study},
	author       = {Li, Qinbin and Diao, Yiqun and Chen, Quan and He, Bingsheng},
	year         = 2022,
	booktitle    = {2022 IEEE 38th International Conference on Data Engineering (ICDE)},
	pages        = {965--978},
	organization = {IEEE}
}
%fednova
@article{wang2020tackling,
	title        = {Tackling the objective inconsistency problem in heterogeneous federated optimization},
	author       = {Wang, Jianyu and Liu, Qinghua and Liang, Hao and Joshi, Gauri and Poor, H Vincent},
	year         = 2020,
	journal      = {Advances in neural information processing systems},
	volume       = 33,
	pages        = {7611--7623}
}
%ida
@incollection{yeganeh2020inverse,
	title        = {Inverse distance aggregation for federated learning with non-iid data},
	author       = {Yeganeh, Yousef and Farshad, Azade and Navab, Nassir and Albarqouni, Shadi},
	year         = 2020,
	booktitle    = {Domain Adaptation and Representation Transfer, and Distributed and Collaborative Learning},
	publisher    = {Springer},
	pages        = {150--159}
}
%mom

%kd
@article{lin2020ensembleFedDF,
	title        = {Ensemble distillation for robust model fusion in federated learning},
	author       = {Lin, Tao and Kong, Lingjing and Stich, Sebastian U and Jaggi, Martin},
	year         = 2020,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 33,
	pages        = {2351--2363}
}
@inproceedings{chen2020fedbe,
	title        = {Fedbe: Making bayesian model ensemble applicable to federated learning},
	author       = {Chen, Hong-You and Chao, Wei-Lun},
	year         = 2021,
	booktitle    = {ICLR}
}
@inproceedings{cho2022heterogeneous,
	title        = {Heterogeneous Ensemble Knowledge Transfer for Training Large Models in Federated Learning},
	author       = {Cho, Yae Jee and Manoel, Andre and Joshi, Gauri and Sim, Robert and Dimitriadis, Dimitrios},
	year         = 2022,
	booktitle    = {IJCAI}
}
@inproceedings{Fedaux,
	title        = {FedAux: An Efficient Framework for Hybrid Federated Learning},
	author       = {Hang Gu and Bin Guo and Jiangtao Wang and Wen Sun and Jiaqi Liu and Sicong Liu and Zhiwen Yu},
	year         = 2022,
	booktitle    = {{IEEE} International Conference on Communications, {ICC} 2022, Seoul, Korea, May 16-20, 2022},
	publisher    = {{IEEE}},
	pages        = {195--200},
	doi          = {10.1109/ICC45855.2022.9839129},
	timestamp    = {Fri, 19 Aug 2022 14:37:27 +0200},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
%abavg
@inproceedings{xiao2021novel,
	title        = {A Novel Server-side Aggregation Strategy for Federated Learning in Non-IID situations},
	author       = {Xiao, Jianhang and Du, Chunhui and Duan, Zijing and Guo, Wei},
	year         = 2021,
	booktitle    = {2021 20th International Symposium on Parallel and Distributed Computing (ISPDC)},
	pages        = {17--24},
	organization = {IEEE}
}
% personalized fl
@article{t2020personalized,
	title        = {Personalized federated learning with moreau envelopes},
	author       = {T Dinh, Canh and Tran, Nguyen and Nguyen, Josh},
	year         = 2020,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 33,
	pages        = {21394--21405}
}
@inproceedings{kulkarni2020survey,
	title        = {Survey of personalization techniques for federated learning},
	author       = {Kulkarni, Viraj and Kulkarni, Milind and Pant, Aniruddha},
	year         = 2020,
	booktitle    = {2020 Fourth World Conference on Smart Trends in Systems, Security and Sustainability (WorldS4)},
	pages        = {794--797},
	organization = {IEEE}
}
@article{hanzely2020lower,
	title        = {Lower bounds and optimal algorithms for personalized federated learning},
	author       = {Hanzely, Filip and Hanzely, Slavom{\'\i}r and Horv{\'a}th, Samuel and Richt{\'a}rik, Peter},
	year         = 2020,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 33,
	pages        = {2304--2315}
}
@inproceedings{li2021ditto,
	title        = {Ditto: Fair and robust federated learning through personalization},
	author       = {Li, Tian and Hu, Shengyuan and Beirami, Ahmad and Smith, Virginia},
	year         = 2021,
	booktitle    = {International Conference on Machine Learning},
	pages        = {6357--6368},
	organization = {PMLR}
}
% similarity clustering
@article{ghosh2019robust,
	title        = {Robust federated learning in a heterogeneous environment},
	author       = {Ghosh, Avishek and Hong, Justin and Yin, Dong and Ramchandran, Kannan},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1906.06629}
}
@inproceedings{briggs2020federated,
	title        = {Federated learning with hierarchical clustering of local updates to improve training on non-IID data},
	author       = {Briggs, Christopher and Fan, Zhong and Andras, Peter},
	year         = 2020,
	booktitle    = {2020 International Joint Conference on Neural Networks (IJCNN)},
	pages        = {1--9},
	organization = {IEEE}
}
@inproceedings{dennis2021heterogeneity,
	title        = {Heterogeneity for the win: One-shot federated clustering},
	author       = {Dennis, Don Kurian and Li, Tian and Smith, Virginia},
	year         = 2021,
	booktitle    = {International Conference on Machine Learning},
	pages        = {2611--2620},
	organization = {PMLR}
}
%data sharing
@article{oh2020mix2fld,
	title        = {Mix2FLD: Downlink federated learning after uplink federated distillation with two-way mixup},
	author       = {Oh, Seungeun and Park, Jihong and Jeong, Eunjeong and Kim, Hyesung and Bennis, Mehdi and Kim, Seong-Lyun},
	year         = 2020,
	journal      = {IEEE Communications Letters},
	publisher    = {IEEE},
	volume       = 24,
	number       = 10,
	pages        = {2211--2215}
}
@article{shin2020xor,
	title        = {Xor mixup: Privacy-preserving data augmentation for one-shot federated learning},
	author       = {Shin, MyungJae and Hwang, Chihoon and Kim, Joongheon and Park, Jihong and Bennis, Mehdi and Kim, Seong-Lyun},
	year         = 2020,
	journal      = {arXiv preprint arXiv:2006.05148}
}
@inproceedings{YoonSHY21,
	title        = {FedMix: Approximation of Mixup under Mean Augmented Federated Learning},
	author       = {Tehrim Yoon and Sumin Shin and Sung Ju Hwang and Eunho Yang},
	year         = 2021,
	booktitle    = {ICLR}
}
%personalized
@inproceedings{chen2021bridging,
	title        = {On bridging generic and personalized federated learning for image classification},
	author       = {Chen, Hong-You and Chao, Wei-Lun},
	year         = 2021,
	booktitle    = {International Conference on Learning Representations}
}
%networks
@inproceedings{he2016deep,
	title        = {Deep residual learning for image recognition},
	author       = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	year         = 2016,
	booktitle    = {Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages        = {770--778}
}
@inproceedings{ma2018shufflenet,
	title        = {Shufflenet v2: Practical guidelines for efficient cnn architecture design},
	author       = {Ma, Ningning and Zhang, Xiangyu and Zheng, Hai-Tao and Sun, Jian},
	year         = 2018,
	booktitle    = {Proceedings of the European conference on computer vision (ECCV)},
	pages        = {116--131}
}
@article{howard2017mobilenets,
	title        = {Mobilenets: Efficient convolutional neural networks for mobile vision applications},
	author       = {Howard, Andrew G and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1704.04861}
}
@article{lecun1998gradient,
	title        = {Gradient-based learning applied to document recognition},
	author       = {LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
	year         = 1998,
	journal      = {Proceedings of the IEEE},
	publisher    = {Ieee},
	volume       = 86,
	number       = 11,
	pages        = {2278--2324}
}
%dataset
@article{krizhevsky2009learning,
	title        = {Learning multiple layers of features from tiny images},
	author       = {Krizhevsky, Alex and Hinton, Geoffrey and others},
	year         = 2009,
	publisher    = {Citeseer}
}
@article{deng2012mnist,
	title        = {The mnist database of handwritten digit images for machine learning research},
	author       = {Deng, Li},
	year         = 2012,
	journal      = {IEEE Signal Processing Magazine},
	publisher    = {IEEE},
	volume       = 29,
	number       = 6,
	pages        = {141--142}
}
%optimizer
%adam
@article{kingma2014adam,
	title        = {Adam: A method for stochastic optimization},
	author       = {Kingma, Diederik P and Ba, Jimmy},
	year         = 2014,
	journal      = {arXiv preprint arXiv:1412.6980}
}
%attack
@article{blanchard2017machine,
	title        = {Machine learning with adversaries: Byzantine tolerant gradient descent},
	author       = {Blanchard, Peva and El Mhamdi, El Mahdi and Guerraoui, Rachid and Stainer, Julien},
	year         = 2017,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 30
}
@article{fung2018mitigating,
	title        = {Mitigating sybils in federated learning poisoning},
	author       = {Fung, Clement and Yoon, Chris JM and Beschastnikh, Ivan},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1808.04866}
}
%defense
@inproceedings{yin2018byzantine,
	title        = {Byzantine-robust distributed learning: Towards optimal statistical rates},
	author       = {Yin, Dong and Chen, Yudong and Kannan, Ramchandran and Bartlett, Peter},
	year         = 2018,
	booktitle    = {International Conference on Machine Learning},
	pages        = {5650--5659},
	organization = {PMLR}
}
@inproceedings{DBLP:conf/iclr/KarimireddyHJ22,
	title        = {Byzantine-Robust Learning on Heterogeneous Datasets via Bucketing},
	author       = {Sai Praneeth Karimireddy and Lie He and Martin Jaggi},
	year         = 2022,
	booktitle    = {The Tenth International Conference on Learning Representations, {ICLR} 2022, Virtual Event, April 25-29, 2022},
	publisher    = {OpenReview.net},
	% url        = {https://openreview.net/forum?id=jXKKDEi5vJt},
	timestamp    = {Sat, 20 Aug 2022 01:15:42 +0200},
	biburl       = {https://dblp.org/rec/conf/iclr/KarimireddyHJ22.bib},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{Fu2021,
	title        = {Attack-Resistant Federated Learning with Residual-based Reweighting},
	author       = {Shuhao Fu and Chulin Xie and Bo Li and Qifeng Chen},
	year         = 2021,
	booktitle    = {AAAI Workshops}
}
@inproceedings{Wan2021,
	title        = {Robust Federated Learning with Attack-Adaptive Aggregation},
	author       = {Ching Pui Wan and Qifeng Chen},
	year         = 2021,
	booktitle    = {IJCAI Workshops}
}
% subspace training
% low dimension
@inproceedings{DBLP:conf/iclr/LiFLY18,
	title        = {Measuring the Intrinsic Dimension of Objective Landscapes},
	author       = {Chunyuan Li and Heerad Farkhoor and Rosanne Liu and Jason Yosinski},
	year         = 2018,
	booktitle    = {6th International Conference on Learning Representations, {ICLR} 2018, Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
	publisher    = {OpenReview.net},
	% url        = {https://openreview.net/forum?id=ryup8-WCW},
	timestamp    = {Thu, 25 Jul 2019 14:25:52 +0200},
	biburl       = {https://dblp.org/rec/conf/iclr/LiFLY18.bib},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
@article{gur2018gradient,
	title        = {Gradient descent happens in a tiny subspace},
	author       = {Gur-Ari, Guy and Roberts, Daniel A and Dyer, Ethan},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1812.04754}
}
@inproceedings{vinyals2012krylov,
	title        = {Krylov subspace descent for deep learning},
	author       = {Vinyals, Oriol and Povey, Daniel},
	year         = 2012,
	booktitle    = {Artificial intelligence and statistics},
	pages        = {1261--1268},
	organization = {PMLR}
}
% traing in subspace
@article{gressmann2020improving,
	title        = {Improving neural network training in low dimensional random bases},
	author       = {Gressmann, Frithjof and Eaton-Rosen, Zach and Luschi, Carlo},
	year         = 2020,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 33,
	pages        = {12140--12150}
}
@article{li2022low,
	title        = {Low Dimensional Trajectory Hypothesis is True: DNNs can be Trained in Tiny Subspaces},
	author       = {Li, Tao and Tan, Lei and Huang, Zhehao and Tao, Qinghua and Liu, Yipeng and Huang, Xiaolin},
	journal      = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	publisher    = {IEEE},
	\
  year     = 2022
}
@inproceedings{li2022subspace,
	title        = {Subspace Adversarial Training},
	author       = {Li, Tao and Wu, Yingwen and Chen, Sizhe and Fang, Kun and Huang, Xiaolin},
	year         = 2022,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {13409--13418}
}
@article{li2022trainable,
	title        = {Trainable Weight Averaging for Fast Convergence and Better Generalization},
	author       = {Li, Tao and Huang, Zhehao and Tao, Qinghua and Wu, Yingwen and Huang, Xiaolin},
	year         = 2022,
	journal      = {arXiv preprint arXiv:2205.13104}
}
% meta learning
@article{jiang2019improving,
	title        = {Improving federated learning personalization via model agnostic meta learning},
	author       = {Jiang, Yihan and Kone{\v{c}}n{\`y}, Jakub and Rush, Keith and Kannan, Sreeram},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1909.12488}
}
@article{li2022federated,
	title        = {Federated meta-learning for spatial-temporal prediction},
	author       = {Li, Wenzhu and Wang, Shuang},
	year         = 2022,
	journal      = {Neural Computing and Applications},
	publisher    = {Springer},
	pages        = {1--20}
}
% attack /defense
@inproceedings{poisoning_attack,
	title        = {Back to the Drawing Board: A Critical Evaluation of Poisoning Attacks on Production Federated Learning},
	author       = {Shejwalkar, Virat and Houmansadr, Amir and Kairouz, Peter and Ramage, Daniel},
	year         = 2022,
	booktitle    = {2022 IEEE Symposium on Security and Privacy (SP)},
	volume       = {},
	number       = {},
	pages        = {1354--1371},
	doi          = {10.1109/SP46214.2022.9833647}
}
@inproceedings{DBLP:conf/iclr/BernsteinZAA19,
	title        = {signSGD with Majority Vote is Communication Efficient and Fault Tolerant},
	author       = {Jeremy Bernstein and Jiawei Zhao and Kamyar Azizzadenesheli and Anima Anandkumar},
	year         = 2019,
	booktitle    = {7th International Conference on Learning Representations, {ICLR} 2019, New Orleans, LA, USA, May 6-9, 2019},
	publisher    = {OpenReview.net},
	% url        = {https://openreview.net/forum?id=BJxhijAcY7},
	timestamp    = {Thu, 25 Jul 2019 14:25:47 +0200},
	biburl       = {https://dblp.org/rec/conf/iclr/BernsteinZAA19.bib},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
% a service of  Schloss Dagstuhl - Leibniz Center for Informatics	homebrowsesearchabout
@inproceedings{guerraoui2018hidden,
	title        = {The hidden vulnerability of distributed learning in byzantium},
	author       = {Guerraoui, Rachid and Rouault, S{\'e}bastien and others},
	year         = 2018,
	booktitle    = {International Conference on Machine Learning},
	pages        = {3521--3530},
	organization = {PMLR}
}
@article{pillutla2019robust,
	title        = {Robust aggregation for federated learning},
	author       = {Pillutla, Krishna and Kakade, Sham M and Harchaoui, Zaid},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1912.13445}
}
@inproceedings{li2019rsa,
	title        = {RSA: Byzantine-robust stochastic aggregation methods for distributed learning from heterogeneous datasets},
	author       = {Li, Liping and Xu, Wei and Chen, Tianyi and Giannakis, Georgios B and Ling, Qing},
	year         = 2019,
	booktitle    = {Proceedings of the AAAI Conference on Artificial Intelligence},
	volume       = 33,
	number       = {01},
	pages        = {1544--1551}
}
@inproceedings{shejwalkar2021manipulating,
	title        = {Manipulating the byzantine: Optimizing model poisoning attacks and defenses for federated learning},
	author       = {Shejwalkar, Virat and Houmansadr, Amir},
	year         = 2021,
	booktitle    = {NDSS}
}
@inproceedings{fltrust,
	title        = {FLTrust: Byzantine-robust Federated Learning via Trust Bootstrapping},
	author       = {Xiaoyu Cao and Minghong Fang and Jia Liu and Neil Zhenqiang Gong},
	year         = 2021,
	booktitle    = {28th Annual Network and Distributed System Security Symposium, {NDSS} 2021, virtually, February 21-25, 2021},
	publisher    = {The Internet Society},
	% url        = {https://www.ndss-symposium.org/ndss-paper/fltrust-byzantine-robust-federated-learning-via-trust-bootstrapping/},
	timestamp    = {Thu, 17 Jun 2021 16:04:48 +0200},
	biburl       = {https://dblp.org/rec/conf/ndss/CaoF0G21.bib},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/KarimireddyHJ22,
	title        = {Byzantine-Robust Learning on Heterogeneous Datasets via Bucketing},
	author       = {Sai Praneeth Karimireddy and Lie He and Martin Jaggi},
	year         = 2022,
	booktitle    = {The Tenth International Conference on Learning Representations, {ICLR} 2022, Virtual Event, April 25-29, 2022},
	publisher    = {OpenReview.net},
	% url        = {https://openreview.net/forum?id=jXKKDEi5vJt},
	timestamp    = {Sat, 20 Aug 2022 01:15:42 +0200},
	biburl       = {https://dblp.org/rec/conf/iclr/KarimireddyHJ22.bib},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
@incollection{lang1995newsweeder,
	title        = {Newsweeder: Learning to filter netnews},
	author       = {Lang, Ken},
	year         = 1995,
	booktitle    = {Machine Learning Proceedings 1995},
	publisher    = {Elsevier},
	pages        = {331--339}
}
%fedmd
@article{li2019fedmd,
	title        = {Fedmd: Heterogenous federated learning via model distillation},
	author       = {Li, Daliang and Wang, Junpu},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1910.03581}
}
@inproceedings{sageflow,
	title        = {Sageflow: Robust Federated Learning against Both Stragglers and Adversaries},
	author       = {Jungwuk Park and Dong{-}Jun Han and Minseok Choi and Jaekyun Moon},
	year         = 2021,
	booktitle    = {Advances in Neural Information Processing Systems 34: Annual Conference on Neural Information Processing Systems 2021, NeurIPS 2021, December 6-14, 2021, virtual},
	pages        = {840--851},
	editor       = {Marc'Aurelio Ranzato and Alina Beygelzimer and Yann N. Dauphin and Percy Liang and Jennifer Wortman Vaughan},
	timestamp    = {Tue, 03 May 2022 16:20:46 +0200},
	biburl       = {https://dblp.org/rec/conf/nips/ParkHCM21.bib},
	bibsource    = {dblp computer science bibliography, https://dblp.org}
}
%  healthcare
@article{rieke2020future,
	title        = {The future of digital health with federated learning},
	author       = {Rieke, Nicola and Hancox, Jonny and Li, Wenqi and Milletari, Fausto and Roth, Holger R and Albarqouni, Shadi and Bakas, Spyridon and Galtier, Mathieu N and Landman, Bennett A and Maier-Hein, Klaus and others},
	year         = 2020,
	journal      = {NPJ digital medicine},
	publisher    = {Nature Publishing Group},
	volume       = 3,
	number       = 1,
	pages        = {1--7}
}
% client bias
@article{wang2021field,
	title        = {A field guide to federated optimization},
	author       = {Wang, Jianyu and Charles, Zachary and Xu, Zheng and Joshi, Gauri and McMahan, H Brendan and Al-Shedivat, Maruan and Andrew, Galen and Avestimehr, Salman and Daly, Katharine and Data, Deepesh and others},
	year         = 2021,
	journal      = {arXiv preprint arXiv:2107.06917}
}
@article{kairouz2021advances,
	title        = {Advances and open problems in federated learning},
	author       = {Kairouz, Peter and McMahan, H Brendan and Avent, Brendan and Bellet, Aur{\'e}lien and Bennis, Mehdi and Bhagoji, Arjun Nitin and Bonawitz, Kallista and Charles, Zachary and Cormode, Graham and Cummings, Rachel and others},
	year         = 2021,
	journal      = {Foundations and Trends{\textregistered} in Machine Learning},
	publisher    = {Now Publishers, Inc.},
	volume       = 14,
	number       = {1--2},
	pages        = {1--210}
}
@article{bonawitz2019towards,
	title        = {Towards federated learning at scale: System design},
	author       = {Bonawitz, Keith and Eichner, Hubert and Grieskamp, Wolfgang and Huba, Dzmitry and Ingerman, Alex and Ivanov, Vladimir and Kiddon, Chloe and Kone{\v{c}}n{\`y}, Jakub and Mazzocchi, Stefano and McMahan, Brendan and others},
	year         = 2019,
	journal      = {Proceedings of Machine Learning and Systems},
	volume       = 1,
	pages        = {374--388}
}
@inproceedings{eichner2019semi,
	title        = {Semi-cyclic stochastic gradient descent},
	author       = {Eichner, Hubert and Koren, Tomer and McMahan, Brendan and Srebro, Nathan and Talwar, Kunal},
	year         = 2019,
	booktitle    = {International Conference on Machine Learning},
	pages        = {1764--1773},
	organization = {PMLR}
}
@article{sheller2020federated,
	title        = {Federated learning in medicine: facilitating multi-institutional collaborations without sharing patient data},
	author       = {Sheller, Micah J and Edwards, Brandon and Reina, G Anthony and Martin, Jason and Pati, Sarthak and Kotrotsou, Aikaterini and Milchenko, Mikhail and Xu, Weilin and Marcus, Daniel and Colen, Rivka R and others},
	year         = 2020,
	journal      = {Scientific reports},
	publisher    = {Nature Publishing Group},
	volume       = 10,
	number       = 1,
	pages        = {1--12}
}
@inproceedings{aggarwal2021fedface,
	title        = {Fedface: Collaborative learning of face recognition model},
	author       = {Aggarwal, Divyansh and Zhou, Jiayu and Jain, Anil K},
	year         = 2021,
	booktitle    = {2021 IEEE International Joint Conference on Biometrics (IJCB)},
	pages        = {1--8},
	organization = {IEEE}
}
@article{li2019convergence,
	title        = {On the convergence of fedavg on non-iid data},
	author       = {Li, Xiang and Huang, Kaixuan and Yang, Wenhao and Wang, Shusen and Zhang, Zhihua},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1907.02189}
}
@article{t2020personalized,
	title        = {Personalized federated learning with moreau envelopes},
	author       = {T Dinh, Canh and Tran, Nguyen and Nguyen, Josh},
	year         = 2020,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 33,
	pages        = {21394--21405}
}
@article{yoon2021fedmix,
	title        = {Fedmix: Approximation of mixup under mean augmented federated learning},
	author       = {Yoon, Tehrim and Shin, Sumin and Hwang, Sung Ju and Yang, Eunho},
	year         = 2021,
	journal      = {arXiv preprint arXiv:2107.00233}
}
@article{zhang2017mixup,
	title        = {mixup: Beyond empirical risk minimization},
	author       = {Zhang, Hongyi and Cisse, Moustapha and Dauphin, Yann N and Lopez-Paz, David},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1710.09412}
}
@online{xiao2017/online,
	title        = {Fashion-MNIST: a Novel Image Dataset for Benchmarking Machine Learning Algorithms},
	author       = {Han Xiao and Kashif Rasul and Roland Vollgraf},
	year         = 2017,
	date         = {2017-08-28},
	eprintclass  = {cs.LG},
	eprinttype   = {arXiv},
	eprint       = {cs.LG/1708.07747}
}
@article{darlow2018cinic,
	title        = {Cinic-10 is not imagenet or cifar-10},
	author       = {Darlow, Luke N and Crowley, Elliot J and Antoniou, Antreas and Storkey, Amos J},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1810.03505}
}
@article{krizhevsky2017imagenet,
	title        = {Imagenet classification with deep convolutional neural networks},
	author       = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
	year         = 2017,
	journal      = {Communications of the ACM},
	publisher    = {AcM New York, NY, USA},
	volume       = 60,
	number       = 6,
	pages        = {84--90}
}
@inproceedings{zhu2021data,
	title        = {Data-free knowledge distillation for heterogeneous federated learning},
	author       = {Zhu, Zhuangdi and Hong, Junyuan and Zhou, Jiayu},
	year         = 2021,
	booktitle    = {International Conference on Machine Learning},
	pages        = {12878--12889},
	organization = {PMLR}
}
@inproceedings{cazenavette2022dataset,
	title        = {Dataset distillation by matching training trajectories},
	author       = {Cazenavette, George and Wang, Tongzhou and Torralba, Antonio and Efros, Alexei A and Zhu, Jun-Yan},
	year         = 2022,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {4750--4759}
}
@article{jochems2017developing,
	title        = {Developing and validating a survival prediction model for NSCLC patients through distributed learning across 3 countries},
	author       = {Jochems, Arthur and Deist, Timo M and El Naqa, Issam and Kessler, Marc and Mayo, Chuck and Reeves, Jackson and Jolly, Shruti and Matuszak, Martha and Ten Haken, Randall and van Soest, Johan and others},
	year         = 2017,
	journal      = {International Journal of Radiation Oncology* Biology* Physics},
	publisher    = {Elsevier},
	volume       = 99,
	number       = 2,
	pages        = {344--352}
}
@article{geiping2020inverting,
	title        = {Inverting gradients-how easy is it to break privacy in federated learning?},
	author       = {Geiping, Jonas and Bauermeister, Hartmut and Dr{\"o}ge, Hannah and Moeller, Michael},
	year         = 2020,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 33,
	pages        = {16937--16947}
}
@inproceedings{yin2021see,
	title        = {See through gradients: Image batch recovery via gradinversion},
	author       = {Yin, Hongxu and Mallya, Arun and Vahdat, Arash and Alvarez, Jose M and Kautz, Jan and Molchanov, Pavlo},
	year         = 2021,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {16337--16346}
}
@inproceedings{zhang2022fine,
	title        = {Fine-tuning global model via data-free knowledge distillation for non-iid federated learning},
	author       = {Zhang, Lin and Shen, Li and Ding, Liang and Tao, Dacheng and Duan, Ling-Yu},
	year         = 2022,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {10174--10183}
}
@article{bonawitz2019towards,
	title        = {Towards federated learning at scale: System design},
	author       = {Bonawitz, Keith and Eichner, Hubert and Grieskamp, Wolfgang and Huba, Dzmitry and Ingerman, Alex and Ivanov, Vladimir and Kiddon, Chloe and Kone{\v{c}}n{\`y}, Jakub and Mazzocchi, Stefano and McMahan, Brendan and others},
	year         = 2019,
	journal      = {Proceedings of Machine Learning and Systems},
	volume       = 1,
	pages        = {374--388}
}
@article{li2020federated,
	title        = {Federated learning: Challenges, methods, and future directions},
	author       = {Li, Tian and Sahu, Anit Kumar and Talwalkar, Ameet and Smith, Virginia},
	year         = 2020,
	journal      = {IEEE Signal Processing Magazine},
	publisher    = {IEEE},
	volume       = 37,
	number       = 3,
	pages        = {50--60}
}
@article{rieke2020future,
	title        = {The future of digital health with federated learning},
	author       = {Rieke, Nicola and Hancox, Jonny and Li, Wenqi and Milletari, Fausto and Roth, Holger R and Albarqouni, Shadi and Bakas, Spyridon and Galtier, Mathieu N and Landman, Bennett A and Maier-Hein, Klaus and others},
	year         = 2020,
	journal      = {NPJ digital medicine},
	publisher    = {Nature Publishing Group},
	volume       = 3,
	number       = 1,
	pages        = {1--7}
}
@article{kairouz2021advances,
	title        = {Advances and open problems in federated learning},
	author       = {Kairouz, Peter and McMahan, H Brendan and Avent, Brendan and Bellet, Aur{\'e}lien and Bennis, Mehdi and Bhagoji, Arjun Nitin and Bonawitz, Kallista and Charles, Zachary and Cormode, Graham and Cummings, Rachel and others},
	year         = 2021,
	journal      = {Foundations and Trends{\textregistered} in Machine Learning},
	publisher    = {Now Publishers, Inc.},
	volume       = 14,
	number       = {1--2},
	pages        = {1--210}
}
@article{li2020federated,
	title        = {Federated optimization in heterogeneous networks},
	author       = {Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
	year         = 2020,
	journal      = {Proceedings of Machine Learning and Systems},
	volume       = 2,
	pages        = {429--450}
}
@inproceedings{zhang2022fine,
	title        = {Fine-tuning global model via data-free knowledge distillation for non-iid federated learning},
	author       = {Zhang, Lin and Shen, Li and Ding, Liang and Tao, Dacheng and Duan, Ling-Yu},
	year         = 2022,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {10174--10183}
}
@article{goodfellow2020generative,
	title        = {Generative adversarial networks},
	author       = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
	year         = 2020,
	journal      = {Communications of the ACM},
	publisher    = {ACM New York, NY, USA},
	volume       = 63,
	number       = 11,
	pages        = {139--144}
}
@article{geiping2020inverting,
	title        = {Inverting gradients-how easy is it to break privacy in federated learning?},
	author       = {Geiping, Jonas and Bauermeister, Hartmut and Dr{\"o}ge, Hannah and Moeller, Michael},
	year         = 2020,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 33,
	pages        = {16937--16947}
}
@inproceedings{yin2021see,
	title        = {See through gradients: Image batch recovery via gradinversion},
	author       = {Yin, Hongxu and Mallya, Arun and Vahdat, Arash and Alvarez, Jose M and Kautz, Jan and Molchanov, Pavlo},
	year         = 2021,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {16337--16346}
}
@article{huang2021evaluating,
	title        = {Evaluating gradient inversion attacks and defenses in federated learning},
	author       = {Huang, Yangsibo and Gupta, Samyak and Song, Zhao and Li, Kai and Arora, Sanjeev},
	year         = 2021,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 34,
	pages        = {7232--7241}
}
@inproceedings{hatamizadeh2022gradvit,
	title        = {Gradvit: Gradient inversion of vision transformers},
	author       = {Hatamizadeh, Ali and Yin, Hongxu and Roth, Holger R and Li, Wenqi and Kautz, Jan and Xu, Daguang and Molchanov, Pavlo},
	year         = 2022,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {10021--10030}
}
@article{jeon2021gradient,
	title        = {Gradient inversion with generative image prior},
	author       = {Jeon, Jinwoo and Lee, Kangwook and Oh, Sewoong and Ok, Jungseul and others},
	year         = 2021,
	journal      = {Advances in Neural Information Processing Systems},
	volume       = 34,
	pages        = {29898--29908}
}
@article{fowl2021robbing,
	title        = {Robbing the fed: Directly obtaining private data in federated learning with modified models},
	author       = {Fowl, Liam and Geiping, Jonas and Czaja, Wojtek and Goldblum, Micah and Goldstein, Tom},
	year         = 2021,
	journal      = {arXiv preprint arXiv:2110.13057}
}
@inproceedings{arpit2017closer,
	title        = {A closer look at memorization in deep networks},
	author       = {Arpit, Devansh and Jastrz{\k{e}}bski, Stanis{\l}aw and Ballas, Nicolas and Krueger, David and Bengio, Emmanuel and Kanwal, Maxinder S and Maharaj, Tegan and Fischer, Asja and Courville, Aaron and Bengio, Yoshua and others},
	year         = 2017,
	booktitle    = {International conference on machine learning},
	pages        = {233--242},
	organization = {PMLR}
}
@article{acar2021federated,
	title        = {Federated learning based on dynamic regularization},
	author       = {Acar, Durmus Alp Emre and Zhao, Yue and Navarro, Ramon Matas and Mattina, Matthew and Whatmough, Paul N and Saligrama, Venkatesh},
	year         = 2021,
	journal      = {arXiv preprint arXiv:2111.04263}
}
@article{xie2022optimizing,
	title        = {Optimizing Server-side Aggregation For Robust Federated Learning via Subspace Training},
	author       = {Yueqi Xie and Weizhong Zhang and Renjie Pi and Fangzhao Wu and Qifeng Chen and Xing Xie and Sunghun Kim},
	year         = 2022,
	journal      = {arXiv preprint arXiv:2211.05554}
}
@article{zhao2021dataset,
	title        = {Dataset Condensation with Gradient Matching.},
	author       = {Zhao, Bo and Mopuri, Konda Reddy and Bilen, Hakan},
	year         = 2021,
	journal      = {ICLR},
	volume       = 1,
	number       = 2,
	pages        = 3
}
@inproceedings{wang2022cafe,
	title        = {Cafe: Learning to condense dataset by aligning features},
	author       = {Wang, Kai and Zhao, Bo and Peng, Xiangyu and Zhu, Zheng and Yang, Shuo and Wang, Shuo and Huang, Guan and Bilen, Hakan and Wang, Xinchao and You, Yang},
	year         = 2022,
	booktitle    = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
	pages        = {12196--12205}
}
@article{dong2022privacy,
	title        = {Privacy for Free: How does Dataset Condensation Help Privacy?},
	author       = {Dong, Tian and Zhao, Bo and Lyu, Lingjuan},
	year         = 2022,
	journal      = {arXiv preprint arXiv:2206.00240}
}



==> cvpr2023-author_kit-v1_1-1/latex/bib_old.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@article{hu2021analysis,
  title={Analysis of biased stochastic gradient descent using sequential semidefinite programs},
  author={Hu, Bin and Seiler, Peter and Lessard, Laurent},
  journal={Mathematical Programming},
  volume={187},
  number={1},
  pages={383--408},
  year={2021},
  publisher={Springer}
}

@article{jacot2018neural,
  title={Neural tangent kernel: Convergence and generalization in neural networks},
  author={Jacot, Arthur and Gabriel, Franck and Hongler, Cl{\'e}ment},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}


@book{wolfgang1998ordinary,
  title={Ordinary differential equations},
  author={Wolfgang, Walter and Walter, Wolfgang and Walter, Wolfgang Ludwig},
  volume={182},
  year={1998},
  publisher={Springer Science \& Business Media}
}


@misc{Authors14,
 author = {FirstName LastName},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture submission ID 324. Supplied as supplemental material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {FirstName LastName},
 title = {Frobnication tutorial},
 note = {Supplied as supplemental material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {FirstName Alpher},
title = {Frobnication},
journal = PAMI,
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@inproceedings{Alpher05,
author = {FirstName Alpher and FirstName Gamow},
title = {Can a computer frobnicate?},
booktitle = CVPR,
pages = {234--778},
year = 2005
}


%%%% Fed background
@article{zhou2021efficient,
  title={Efficient neural network training via forward and backward propagation sparsification},
  author={Zhou, Xiao and Zhang, Weizhong and Chen, Zonghao and Diao, Shizhe and Zhang, Tong},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={15216--15229},
  year={2021}
}

@inproceedings{xie2020zeno++,
  title={Zeno++: Robust fully asynchronous SGD},
  author={Xie, Cong and Koyejo, Sanmi and Gupta, Indranil},
  booktitle={International Conference on Machine Learning},
  pages={10495--10503},
  year={2020},
  organization={PMLR}
}

@inproceedings{xie2019zeno,
  title={Zeno: Distributed stochastic gradient descent with suspicion-based fault-tolerance},
  author={Xie, Cong and Koyejo, Sanmi and Gupta, Indranil},
  booktitle={International Conference on Machine Learning},
  pages={6893--6901},
  year={2019},
  organization={PMLR}
}

@book{wainwright2019high,
  title={High-dimensional statistics: A non-asymptotic viewpoint},
  author={Wainwright, Martin J},
  volume={48},
  year={2019},
  publisher={Cambridge University Press}
}
@article{polyak1964gradient,
  title={Gradient methods for solving equations and inequalities},
  author={Polyak, Boris T},
  journal={USSR Computational Mathematics and Mathematical Physics},
  volume={4},
  number={6},
  pages={17--32},
  year={1964},
  publisher={Elsevier}
}

@article{kuditipudi2019explaining,
  title={Explaining landscape connectivity of low-cost solutions for multilayer nets},
  author={Kuditipudi, Rohith and Wang, Xiang and Lee, Holden and Zhang, Yi and Li, Zhiyuan and Hu, Wei and Ge, Rong and Arora, Sanjeev},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{stich2018local,
  title={Local SGD Converges Fast and Communicates Little},
  author={Stich, Sebastian U},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{li2020convergence,
  title={On the Convergence of FedAvg on Non-IID Data},
  author={Li, Xiang and Huang, Kaixuan and Yang, Wenhao and Wang, Shusen and Zhang, Zhihua},
  booktitle={International Conference on Learning Representations},
  year={2020}
}

@article{hoffman2018algorithms,
  title={Algorithms and theory for multiple-source adaptation},
  author={Hoffman, Judy and Mohri, Mehryar and Zhang, Ningshan},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}

@article{konevcny2016federated,
  title={Federated learning: Strategies for improving communication efficiency},
  author={Kone{\v{c}}n{\`y}, Jakub and McMahan, H Brendan and Yu, Felix X and Richt{\'a}rik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
  journal={arXiv preprint arXiv:1610.05492},
  year={2016}
}
@article{yang2019federated,
  title={Federated machine learning: Concept and applications},
  author={Yang, Qiang and Liu, Yang and Chen, Tianjian and Tong, Yongxin},
  journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
  volume={10},
  number={2},
  pages={1--19},
  year={2019},
  publisher={ACM New York, NY, USA}
}


%noniid
@article{hsu2019measuring,
  title={Measuring the effects of non-identical data distribution for federated visual classification},
  author={Hsu, Tzu-Ming Harry and Qi, Hang and Brown, Matthew},
  journal={arXiv preprint arXiv:1909.06335},
  year={2019}
}
%fedavg convergence
@inproceedings{mcmahan2017communication,
  title={Communication-efficient learning of deep networks from decentralized data},
  author={McMahan, H Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and others},
  booktitle={AISTATS},
  year={2017}
}

@article{sahu2018convergence,
  title={On the convergence of federated optimization in heterogeneous networks},
  author={Sahu, Anit Kumar and Li, Tian and Sanjabi, Maziar and Zaheer, Manzil and Talwalkar, Ameet and Smith, Virginia},
  journal={arXiv preprint arXiv:1812.06127},
  year={2018}
}

@inproceedings{zinkevich2010parallelized,
  title={Parallelized stochastic gradient descent},
  author={Zinkevich, Martin and Weimer, Markus and Li, Lihong and Smola, Alex J},
  booktitle={NIPS},
  year={2010}
}

@article{zhou2017convergence,
  title={On the convergence properties of a $ K $-step averaging stochastic gradient descent algorithm for nonconvex optimization},
  author={Zhou, Fan and Cong, Guojing},
  journal={arXiv preprint arXiv:1708.01012},
  year={2017}
}

%drift 
@article{zhao2018federated,
  title={Federated learning with non-iid data},
  author={Zhao, Yue and Li, Meng and Lai, Liangzhen and Suda, Naveen and Civin, Damon and Chandra, Vikas},
  journal={arXiv preprint arXiv:1806.00582},
  year={2018}
}

@inproceedings{karimireddy2019scaffold,
  title={SCAFFOLD: Stochastic controlled averaging for on-device federated learning},
  author={Karimireddy, Sai Praneeth and Kale, Satyen and Mohri, Mehryar and Reddi, Sashank J and Stich, Sebastian U and Suresh, Ananda Theertha},
  booktitle={ICML},
  year={2020}
}


@inproceedings{Acar2021Dyn,
  author    = {Durmus Alp Emre Acar and
               Yue Zhao and
               Ramon Matas Navarro and
               Matthew Mattina and
               Paul N. Whatmough and
               Venkatesh Saligrama},
  title     = {Federated Learning Based on Dynamic Regularization},
  booktitle = {ICLR},
  year      = {2021},
  timestamp = {Thu, 14 Oct 2021 10:00:36 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/AcarZNMWS21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

%fedprox
@inproceedings{li2020federated,
  title={Federated optimization in heterogeneous networks},
  author={Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
  booktitle={MLSys},
  year={2020}
}


@inproceedings{li2019feddane,
  title={Feddane: A federated newton-type method},
  author={Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smithy, Virginia},
  booktitle={2019 53rd Asilomar Conference on Signals, Systems, and Computers},
  pages={1227--1231},
  year={2019},
  organization={IEEE}
}
@article{yao2019federated,
  title={Federated Learning with Unbiased Gradient Aggregation and Controllable Meta Updating},
  author={Yao, Xin and Huang, Tianchi and Zhang, Rui-Xiao and Li, Ruiyu and Sun, Lifeng},
  journal={arXiv preprint arXiv:1910.08234},
  year={2019}
}

@inproceedings{li2021model,
  title={Model-contrastive federated learning},
  author={Li, Qinbin and He, Bingsheng and Song, Dawn},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10713--10722},
  year={2021}
}

%model connectivity
@article{garipov2018loss,
  title={Loss surfaces, mode connectivity, and fast ensembling of dnns},
  author={Garipov, Timur and Izmailov, Pavel and Podoprikhin, Dmitrii and Vetrov, Dmitry P and Wilson, Andrew G},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}
@inproceedings{draxler2018essentially,
  title={Essentially no barriers in neural network energy landscape},
  author={Draxler, Felix and Veschgini, Kambis and Salmhofer, Manfred and Hamprecht, Fred},
  booktitle={International conference on machine learning},
  pages={1309--1318},
  year={2018},
  organization={PMLR}
}
%server agg
% good perform fedavg
@inproceedings{li2022federated,
  title={Federated learning on non-iid data silos: An experimental study},
  author={Li, Qinbin and Diao, Yiqun and Chen, Quan and He, Bingsheng},
  booktitle={2022 IEEE 38th International Conference on Data Engineering (ICDE)},
  pages={965--978},
  year={2022},
  organization={IEEE}
}


%fednova
@article{wang2020tackling,
  title={Tackling the objective inconsistency problem in heterogeneous federated optimization},
  author={Wang, Jianyu and Liu, Qinghua and Liang, Hao and Joshi, Gauri and Poor, H Vincent},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={7611--7623},
  year={2020}
}

%ida
@incollection{yeganeh2020inverse,
  title={Inverse distance aggregation for federated learning with non-iid data},
  author={Yeganeh, Yousef and Farshad, Azade and Navab, Nassir and Albarqouni, Shadi},
  booktitle={Domain Adaptation and Representation Transfer, and Distributed and Collaborative Learning},
  pages={150--159},
  year={2020},
  publisher={Springer}
}
%mom

%kd
@article{lin2020ensembleFedDF,
  title={Ensemble distillation for robust model fusion in federated learning},
  author={Lin, Tao and Kong, Lingjing and Stich, Sebastian U and Jaggi, Martin},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={2351--2363},
  year={2020}
}
@inproceedings{chen2020fedbe,
  title={Fedbe: Making bayesian model ensemble applicable to federated learning},
  author={Chen, Hong-You and Chao, Wei-Lun},
  booktitle={ICLR},
  year={2021}
}

@inproceedings{cho2022heterogeneous,
  title={Heterogeneous Ensemble Knowledge Transfer for Training Large Models in Federated Learning},
  author={Cho, Yae Jee and Manoel, Andre and Joshi, Gauri and Sim, Robert and Dimitriadis, Dimitrios},
  booktitle={IJCAI},
  year={2022}
}
@inproceedings{Fedaux,
  author    = {Hang Gu and
               Bin Guo and
               Jiangtao Wang and
               Wen Sun and
               Jiaqi Liu and
               Sicong Liu and
               Zhiwen Yu},
  title     = {FedAux: An Efficient Framework for Hybrid Federated Learning},
  booktitle = {{IEEE} International Conference on Communications, {ICC} 2022, Seoul,
               Korea, May 16-20, 2022},
  pages     = {195--200},
  publisher = {{IEEE}},
  year      = {2022},
  doi       = {10.1109/ICC45855.2022.9839129},
  timestamp = {Fri, 19 Aug 2022 14:37:27 +0200},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
%abavg
@inproceedings{xiao2021novel,
  title={A Novel Server-side Aggregation Strategy for Federated Learning in Non-IID situations},
  author={Xiao, Jianhang and Du, Chunhui and Duan, Zijing and Guo, Wei},
  booktitle={2021 20th International Symposium on Parallel and Distributed Computing (ISPDC)},
  pages={17--24},
  year={2021},
  organization={IEEE}
}

% personalized fl
@article{t2020personalized,
  title={Personalized federated learning with moreau envelopes},
  author={T Dinh, Canh and Tran, Nguyen and Nguyen, Josh},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={21394--21405},
  year={2020}
}
@inproceedings{kulkarni2020survey,
  title={Survey of personalization techniques for federated learning},
  author={Kulkarni, Viraj and Kulkarni, Milind and Pant, Aniruddha},
  booktitle={2020 Fourth World Conference on Smart Trends in Systems, Security and Sustainability (WorldS4)},
  pages={794--797},
  year={2020},
  organization={IEEE}
}
@article{hanzely2020lower,
  title={Lower bounds and optimal algorithms for personalized federated learning},
  author={Hanzely, Filip and Hanzely, Slavom{\'\i}r and Horv{\'a}th, Samuel and Richt{\'a}rik, Peter},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={2304--2315},
  year={2020}
}

@inproceedings{li2021ditto,
  title={Ditto: Fair and robust federated learning through personalization},
  author={Li, Tian and Hu, Shengyuan and Beirami, Ahmad and Smith, Virginia},
  booktitle={International Conference on Machine Learning},
  pages={6357--6368},
  year={2021},
  organization={PMLR}
}
% similarity clustering
@article{ghosh2019robust,
  title={Robust federated learning in a heterogeneous environment},
  author={Ghosh, Avishek and Hong, Justin and Yin, Dong and Ramchandran, Kannan},
  journal={arXiv preprint arXiv:1906.06629},
  year={2019}
}
@inproceedings{briggs2020federated,
  title={Federated learning with hierarchical clustering of local updates to improve training on non-IID data},
  author={Briggs, Christopher and Fan, Zhong and Andras, Peter},
  booktitle={2020 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--9},
  year={2020},
  organization={IEEE}
}
@inproceedings{dennis2021heterogeneity,
  title={Heterogeneity for the win: One-shot federated clustering},
  author={Dennis, Don Kurian and Li, Tian and Smith, Virginia},
  booktitle={International Conference on Machine Learning},
  pages={2611--2620},
  year={2021},
  organization={PMLR}
}

%data sharing
@article{oh2020mix2fld,
  title={Mix2FLD: Downlink federated learning after uplink federated distillation with two-way mixup},
  author={Oh, Seungeun and Park, Jihong and Jeong, Eunjeong and Kim, Hyesung and Bennis, Mehdi and Kim, Seong-Lyun},
  journal={IEEE Communications Letters},
  volume={24},
  number={10},
  pages={2211--2215},
  year={2020},
  publisher={IEEE}
}


@article{shin2020xor,
  title={Xor mixup: Privacy-preserving data augmentation for one-shot federated learning},
  author={Shin, MyungJae and Hwang, Chihoon and Kim, Joongheon and Park, Jihong and Bennis, Mehdi and Kim, Seong-Lyun},
  journal={arXiv preprint arXiv:2006.05148},
  year={2020}
}

@inproceedings{YoonSHY21,
  author    = {Tehrim Yoon and
               Sumin Shin and
               Sung Ju Hwang and
               Eunho Yang},
  title     = {FedMix: Approximation of Mixup under Mean Augmented Federated Learning},
  booktitle = {ICLR},
  year      = {2021},
}


%personalized
@inproceedings{chen2021bridging,
  title={On bridging generic and personalized federated learning for image classification},
  author={Chen, Hong-You and Chao, Wei-Lun},
  booktitle={International Conference on Learning Representations},
  year={2021}
}


%networks
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}



@inproceedings{ma2018shufflenet,
  title={Shufflenet v2: Practical guidelines for efficient cnn architecture design},
  author={Ma, Ningning and Zhang, Xiangyu and Zheng, Hai-Tao and Sun, Jian},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={116--131},
  year={2018}
}
@article{howard2017mobilenets,
  title={Mobilenets: Efficient convolutional neural networks for mobile vision applications},
  author={Howard, Andrew G and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
  journal={arXiv preprint arXiv:1704.04861},
  year={2017}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}
%dataset
@article{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  year={2009},
  publisher={Citeseer}
}

@article{deng2012mnist,
  title={The mnist database of handwritten digit images for machine learning research},
  author={Deng, Li},
  journal={IEEE Signal Processing Magazine},
  volume={29},
  number={6},
  pages={141--142},
  year={2012},
  publisher={IEEE}
}
%optimizer
%adam
@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

%attack
@article{blanchard2017machine,
  title={Machine learning with adversaries: Byzantine tolerant gradient descent},
  author={Blanchard, Peva and El Mhamdi, El Mahdi and Guerraoui, Rachid and Stainer, Julien},
  journal={Advances in Neural Information Processing Systems},
  volume={30},
  year={2017}
}
@article{fung2018mitigating,
  title={Mitigating sybils in federated learning poisoning},
  author={Fung, Clement and Yoon, Chris JM and Beschastnikh, Ivan},
  journal={arXiv preprint arXiv:1808.04866},
  year={2018}
}

%defense
@inproceedings{yin2018byzantine,
  title={Byzantine-robust distributed learning: Towards optimal statistical rates},
  author={Yin, Dong and Chen, Yudong and Kannan, Ramchandran and Bartlett, Peter},
  booktitle={International Conference on Machine Learning},
  pages={5650--5659},
  year={2018},
  organization={PMLR}
}

@inproceedings{DBLP:conf/iclr/KarimireddyHJ22,
  author    = {Sai Praneeth Karimireddy and
               Lie He and
               Martin Jaggi},
  title     = {Byzantine-Robust Learning on Heterogeneous Datasets via Bucketing},
  booktitle = {The Tenth International Conference on Learning Representations, {ICLR}
               2022, Virtual Event, April 25-29, 2022},
  publisher = {OpenReview.net},
  year      = {2022},
  % url       = {https://openreview.net/forum?id=jXKKDEi5vJt},
  timestamp = {Sat, 20 Aug 2022 01:15:42 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/KarimireddyHJ22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Fu2021,
  author    = {Shuhao Fu and
               Chulin Xie and
               Bo Li and
               Qifeng Chen},
  title     = {Attack-Resistant Federated Learning with Residual-based Reweighting},
  booktitle   = {AAAI Workshops},
  year      = {2021},
}

@inproceedings{Wan2021,
  author    = {Ching Pui Wan and
               Qifeng Chen},
  title     = {Robust Federated Learning with Attack-Adaptive Aggregation},
  booktitle   = {IJCAI Workshops},
  year      = {2021},
}


% subspace training
% low dimension
@inproceedings{DBLP:conf/iclr/LiFLY18,
  author    = {Chunyuan Li and
               Heerad Farkhoor and
               Rosanne Liu and
               Jason Yosinski},
  title     = {Measuring the Intrinsic Dimension of Objective Landscapes},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  % url       = {https://openreview.net/forum?id=ryup8-WCW},
  timestamp = {Thu, 25 Jul 2019 14:25:52 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/LiFLY18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{gur2018gradient,
  title={Gradient descent happens in a tiny subspace},
  author={Gur-Ari, Guy and Roberts, Daniel A and Dyer, Ethan},
  journal={arXiv preprint arXiv:1812.04754},
  year={2018}
}
@inproceedings{vinyals2012krylov,
  title={Krylov subspace descent for deep learning},
  author={Vinyals, Oriol and Povey, Daniel},
  booktitle={Artificial intelligence and statistics},
  pages={1261--1268},
  year={2012},
  organization={PMLR}
}
% traing in subspace
@article{gressmann2020improving,
  title={Improving neural network training in low dimensional random bases},
  author={Gressmann, Frithjof and Eaton-Rosen, Zach and Luschi, Carlo},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={12140--12150},
  year={2020}
}

@article{li2022low, 
  title={Low Dimensional Trajectory Hypothesis is True: DNNs can be Trained in Tiny Subspaces}, 
  author={Li, Tao and Tan, Lei and Huang, Zhehao and Tao, Qinghua and Liu, Yipeng and Huang, Xiaolin}, 
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, \
  year={2022}, 
  publisher={IEEE} 
}

@inproceedings{li2022subspace,
  title={Subspace Adversarial Training},
  author={Li, Tao and Wu, Yingwen and Chen, Sizhe and Fang, Kun and Huang, Xiaolin},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13409--13418},
  year={2022}
}

@article{li2022trainable,
  title={Trainable Weight Averaging for Fast Convergence and Better Generalization},
  author={Li, Tao and Huang, Zhehao and Tao, Qinghua and Wu, Yingwen and Huang, Xiaolin},
  journal={arXiv preprint arXiv:2205.13104},
  year={2022}
}

% meta learning
@article{jiang2019improving,
  title={Improving federated learning personalization via model agnostic meta learning},
  author={Jiang, Yihan and Kone{\v{c}}n{\`y}, Jakub and Rush, Keith and Kannan, Sreeram},
  journal={arXiv preprint arXiv:1909.12488},
  year={2019}
}
@article{li2022federated,
  title={Federated meta-learning for spatial-temporal prediction},
  author={Li, Wenzhu and Wang, Shuang},
  journal={Neural Computing and Applications},
  pages={1--20},
  year={2022},
  publisher={Springer}
}

% attack /defense
@INPROCEEDINGS{poisoning_attack,
  author={Shejwalkar, Virat and Houmansadr, Amir and Kairouz, Peter and Ramage, Daniel},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)}, 
  title={Back to the Drawing Board: A Critical Evaluation of Poisoning Attacks on Production Federated Learning}, 
  year={2022},
  volume={},
  number={},
  pages={1354-1371},
  doi={10.1109/SP46214.2022.9833647}}

  @inproceedings{DBLP:conf/iclr/BernsteinZAA19,
  author    = {Jeremy Bernstein and
               Jiawei Zhao and
               Kamyar Azizzadenesheli and
               Anima Anandkumar},
  title     = {signSGD with Majority Vote is Communication Efficient and Fault Tolerant},
  booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  publisher = {OpenReview.net},
  year      = {2019},
  % url       = {https://openreview.net/forum?id=BJxhijAcY7},
  timestamp = {Thu, 25 Jul 2019 14:25:47 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/BernsteinZAA19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
% a service of  Schloss Dagstuhl - Leibniz Center for Informatics	homebrowsesearchabout



@inproceedings{guerraoui2018hidden,
  title={The hidden vulnerability of distributed learning in byzantium},
  author={Guerraoui, Rachid and Rouault, S{\'e}bastien and others},
  booktitle={International Conference on Machine Learning},
  pages={3521--3530},
  year={2018},
  organization={PMLR}
}

@article{pillutla2019robust,
  title={Robust aggregation for federated learning},
  author={Pillutla, Krishna and Kakade, Sham M and Harchaoui, Zaid},
  journal={arXiv preprint arXiv:1912.13445},
  year={2019}
}

@inproceedings{li2019rsa,
  title={RSA: Byzantine-robust stochastic aggregation methods for distributed learning from heterogeneous datasets},
  author={Li, Liping and Xu, Wei and Chen, Tianyi and Giannakis, Georgios B and Ling, Qing},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={1544--1551},
  year={2019}
}

@inproceedings{shejwalkar2021manipulating,
  title={Manipulating the byzantine: Optimizing model poisoning attacks and defenses for federated learning},
  author={Shejwalkar, Virat and Houmansadr, Amir},
  booktitle={NDSS},
  year={2021}
}

@inproceedings{fltrust,
  author    = {Xiaoyu Cao and
               Minghong Fang and
               Jia Liu and
               Neil Zhenqiang Gong},
  title     = {FLTrust: Byzantine-robust Federated Learning via Trust Bootstrapping},
  booktitle = {28th Annual Network and Distributed System Security Symposium, {NDSS}
               2021, virtually, February 21-25, 2021},
  publisher = {The Internet Society},
  year      = {2021},
  % url       = {https://www.ndss-symposium.org/ndss-paper/fltrust-byzantine-robust-federated-learning-via-trust-bootstrapping/},
  timestamp = {Thu, 17 Jun 2021 16:04:48 +0200},
  biburl    = {https://dblp.org/rec/conf/ndss/CaoF0G21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/iclr/KarimireddyHJ22,
  author    = {Sai Praneeth Karimireddy and
               Lie He and
               Martin Jaggi},
  title     = {Byzantine-Robust Learning on Heterogeneous Datasets via Bucketing},
  booktitle = {The Tenth International Conference on Learning Representations, {ICLR}
               2022, Virtual Event, April 25-29, 2022},
  publisher = {OpenReview.net},
  year      = {2022},
  % url       = {https://openreview.net/forum?id=jXKKDEi5vJt},
  timestamp = {Sat, 20 Aug 2022 01:15:42 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/KarimireddyHJ22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@incollection{lang1995newsweeder,
  title={Newsweeder: Learning to filter netnews},
  author={Lang, Ken},
  booktitle={Machine Learning Proceedings 1995},
  pages={331--339},
  year={1995},
  publisher={Elsevier}
}


%fedmd
@article{li2019fedmd,
  title={Fedmd: Heterogenous federated learning via model distillation},
  author={Li, Daliang and Wang, Junpu},
  journal={arXiv preprint arXiv:1910.03581},
  year={2019}
}

@inproceedings{sageflow,
  author    = {Jungwuk Park and
               Dong{-}Jun Han and
               Minseok Choi and
               Jaekyun Moon},
  editor    = {Marc'Aurelio Ranzato and
               Alina Beygelzimer and
               Yann N. Dauphin and
               Percy Liang and
               Jennifer Wortman Vaughan},
  title     = {Sageflow: Robust Federated Learning against Both Stragglers and Adversaries},
  booktitle = {Advances in Neural Information Processing Systems 34: Annual Conference
               on Neural Information Processing Systems 2021, NeurIPS 2021, December
               6-14, 2021, virtual},
  pages     = {840--851},
  year      = {2021},
  timestamp = {Tue, 03 May 2022 16:20:46 +0200},
  biburl    = {https://dblp.org/rec/conf/nips/ParkHCM21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

%  healthcare
@article{rieke2020future,
  title={The future of digital health with federated learning},
  author={Rieke, Nicola and Hancox, Jonny and Li, Wenqi and Milletari, Fausto and Roth, Holger R and Albarqouni, Shadi and Bakas, Spyridon and Galtier, Mathieu N and Landman, Bennett A and Maier-Hein, Klaus and others},
  journal={NPJ digital medicine},
  volume={3},
  number={1},
  pages={1--7},
  year={2020},
  publisher={Nature Publishing Group}
}

% client bias
@article{wang2021field,
  title={A field guide to federated optimization},
  author={Wang, Jianyu and Charles, Zachary and Xu, Zheng and Joshi, Gauri and McMahan, H Brendan and Al-Shedivat, Maruan and Andrew, Galen and Avestimehr, Salman and Daly, Katharine and Data, Deepesh and others},
  journal={arXiv preprint arXiv:2107.06917},
  year={2021}
}

@article{kairouz2021advances,
  title={Advances and open problems in federated learning},
  author={Kairouz, Peter and McMahan, H Brendan and Avent, Brendan and Bellet, Aur{\'e}lien and Bennis, Mehdi and Bhagoji, Arjun Nitin and Bonawitz, Kallista and Charles, Zachary and Cormode, Graham and Cummings, Rachel and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={14},
  number={1--2},
  pages={1--210},
  year={2021},
  publisher={Now Publishers, Inc.}
}

@article{bonawitz2019towards,
  title={Towards federated learning at scale: System design},
  author={Bonawitz, Keith and Eichner, Hubert and Grieskamp, Wolfgang and Huba, Dzmitry and Ingerman, Alex and Ivanov, Vladimir and Kiddon, Chloe and Kone{\v{c}}n{\`y}, Jakub and Mazzocchi, Stefano and McMahan, Brendan and others},
  journal={Proceedings of Machine Learning and Systems},
  volume={1},
  pages={374--388},
  year={2019}
}

@inproceedings{eichner2019semi,
  title={Semi-cyclic stochastic gradient descent},
  author={Eichner, Hubert and Koren, Tomer and McMahan, Brendan and Srebro, Nathan and Talwar, Kunal},
  booktitle={International Conference on Machine Learning},
  pages={1764--1773},
  year={2019},
  organization={PMLR}
}
@article{sheller2020federated,
  title={Federated learning in medicine: facilitating multi-institutional collaborations without sharing patient data},
  author={Sheller, Micah J and Edwards, Brandon and Reina, G Anthony and Martin, Jason and Pati, Sarthak and Kotrotsou, Aikaterini and Milchenko, Mikhail and Xu, Weilin and Marcus, Daniel and Colen, Rivka R and others},
  journal={Scientific reports},
  volume={10},
  number={1},
  pages={1--12},
  year={2020},
  publisher={Nature Publishing Group}
}

@inproceedings{aggarwal2021fedface,
  title={Fedface: Collaborative learning of face recognition model},
  author={Aggarwal, Divyansh and Zhou, Jiayu and Jain, Anil K},
  booktitle={2021 IEEE International Joint Conference on Biometrics (IJCB)},
  pages={1--8},
  year={2021},
  organization={IEEE}
}
@article{li2019convergence,
  title={On the convergence of fedavg on non-iid data},
  author={Li, Xiang and Huang, Kaixuan and Yang, Wenhao and Wang, Shusen and Zhang, Zhihua},
  journal={arXiv preprint arXiv:1907.02189},
  year={2019}
}
@article{t2020personalized,
  title={Personalized federated learning with moreau envelopes},
  author={T Dinh, Canh and Tran, Nguyen and Nguyen, Josh},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={21394--21405},
  year={2020}
}
@article{yoon2021fedmix,
  title={Fedmix: Approximation of mixup under mean augmented federated learning},
  author={Yoon, Tehrim and Shin, Sumin and Hwang, Sung Ju and Yang, Eunho},
  journal={arXiv preprint arXiv:2107.00233},
  year={2021}
}
@article{zhang2017mixup,
  title={mixup: Beyond empirical risk minimization},
  author={Zhang, Hongyi and Cisse, Moustapha and Dauphin, Yann N and Lopez-Paz, David},
  journal={arXiv preprint arXiv:1710.09412},
  year={2017}
}
@online{xiao2017/online,
  author       = {Han Xiao and Kashif Rasul and Roland Vollgraf},
  title        = {Fashion-MNIST: a Novel Image Dataset for Benchmarking Machine Learning Algorithms},
  date         = {2017-08-28},
  year         = {2017},
  eprintclass  = {cs.LG},
  eprinttype   = {arXiv},
  eprint       = {cs.LG/1708.07747},
}
@article{darlow2018cinic,
  title={Cinic-10 is not imagenet or cifar-10},
  author={Darlow, Luke N and Crowley, Elliot J and Antoniou, Antreas and Storkey, Amos J},
  journal={arXiv preprint arXiv:1810.03505},
  year={2018}
}
@article{krizhevsky2017imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Communications of the ACM},
  volume={60},
  number={6},
  pages={84--90},
  year={2017},
  publisher={AcM New York, NY, USA}
}
@inproceedings{zhu2021data,
  title={Data-free knowledge distillation for heterogeneous federated learning},
  author={Zhu, Zhuangdi and Hong, Junyuan and Zhou, Jiayu},
  booktitle={International Conference on Machine Learning},
  pages={12878--12889},
  year={2021},
  organization={PMLR}
}
@inproceedings{cazenavette2022dataset,
  title={Dataset distillation by matching training trajectories},
  author={Cazenavette, George and Wang, Tongzhou and Torralba, Antonio and Efros, Alexei A and Zhu, Jun-Yan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4750--4759},
  year={2022}
}
@article{jochems2017developing,
  title={Developing and validating a survival prediction model for NSCLC patients through distributed learning across 3 countries},
  author={Jochems, Arthur and Deist, Timo M and El Naqa, Issam and Kessler, Marc and Mayo, Chuck and Reeves, Jackson and Jolly, Shruti and Matuszak, Martha and Ten Haken, Randall and van Soest, Johan and others},
  journal={International Journal of Radiation Oncology* Biology* Physics},
  volume={99},
  number={2},
  pages={344--352},
  year={2017},
  publisher={Elsevier}
}
@article{geiping2020inverting,
  title={Inverting gradients-how easy is it to break privacy in federated learning?},
  author={Geiping, Jonas and Bauermeister, Hartmut and Dr{\"o}ge, Hannah and Moeller, Michael},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={16937--16947},
  year={2020}
}
@inproceedings{yin2021see,
  title={See through gradients: Image batch recovery via gradinversion},
  author={Yin, Hongxu and Mallya, Arun and Vahdat, Arash and Alvarez, Jose M and Kautz, Jan and Molchanov, Pavlo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={16337--16346},
  year={2021}
}
@inproceedings{zhang2022fine,
  title={Fine-tuning global model via data-free knowledge distillation for non-iid federated learning},
  author={Zhang, Lin and Shen, Li and Ding, Liang and Tao, Dacheng and Duan, Ling-Yu},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10174--10183},
  year={2022}
}
@article{goodfellow2020generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Communications of the ACM},
  volume={63},
  number={11},
  pages={139--144},
  year={2020},
  publisher={ACM New York, NY, USA}
}
@article{geiping2020inverting,
  title={Inverting gradients-how easy is it to break privacy in federated learning?},
  author={Geiping, Jonas and Bauermeister, Hartmut and Dr{\"o}ge, Hannah and Moeller, Michael},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={16937--16947},
  year={2020}
}
@inproceedings{yin2021see,
  title={See through gradients: Image batch recovery via gradinversion},
  author={Yin, Hongxu and Mallya, Arun and Vahdat, Arash and Alvarez, Jose M and Kautz, Jan and Molchanov, Pavlo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={16337--16346},
  year={2021}
}
@article{huang2021evaluating,
  title={Evaluating gradient inversion attacks and defenses in federated learning},
  author={Huang, Yangsibo and Gupta, Samyak and Song, Zhao and Li, Kai and Arora, Sanjeev},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={7232--7241},
  year={2021}
}
@inproceedings{hatamizadeh2022gradvit,
  title={Gradvit: Gradient inversion of vision transformers},
  author={Hatamizadeh, Ali and Yin, Hongxu and Roth, Holger R and Li, Wenqi and Kautz, Jan and Xu, Daguang and Molchanov, Pavlo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10021--10030},
  year={2022}
}
@article{jeon2021gradient,
  title={Gradient inversion with generative image prior},
  author={Jeon, Jinwoo and Lee, Kangwook and Oh, Sewoong and Ok, Jungseul and others},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={29898--29908},
  year={2021}
}
@article{fowl2021robbing,
  title={Robbing the fed: Directly obtaining private data in federated learning with modified models},
  author={Fowl, Liam and Geiping, Jonas and Czaja, Wojtek and Goldblum, Micah and Goldstein, Tom},
  journal={arXiv preprint arXiv:2110.13057},
  year={2021}
}
@inproceedings{arpit2017closer,
  title={A closer look at memorization in deep networks},
  author={Arpit, Devansh and Jastrz{\k{e}}bski, Stanis{\l}aw and Ballas, Nicolas and Krueger, David and Bengio, Emmanuel and Kanwal, Maxinder S and Maharaj, Tegan and Fischer, Asja and Courville, Aaron and Bengio, Yoshua and others},
  booktitle={International conference on machine learning},
  pages={233--242},
  year={2017},
  organization={PMLR}
}
@article{acar2021federated,
  title={Federated learning based on dynamic regularization},
  author={Acar, Durmus Alp Emre and Zhao, Yue and Navarro, Ramon Matas and Mattina, Matthew and Whatmough, Paul N and Saligrama, Venkatesh},
  journal={arXiv preprint arXiv:2111.04263},
  year={2021}
}
@article{xie2022optimizing,
      title={Optimizing Server-side Aggregation For Robust Federated Learning via Subspace Training}, 
      author={Yueqi Xie and Weizhong Zhang and Renjie Pi and Fangzhao Wu and Qifeng Chen and Xing Xie and Sunghun Kim},
      year={2022},
      journal={arXiv preprint arXiv:2211.05554},
}
@article{zhao2021dataset,
  title={Dataset Condensation with Gradient Matching.},
  author={Zhao, Bo and Mopuri, Konda Reddy and Bilen, Hakan},
  journal={ICLR},
  volume={1},
  number={2},
  pages={3},
  year={2021}
}
@inproceedings{wang2022cafe,
  title={Cafe: Learning to condense dataset by aligning features},
  author={Wang, Kai and Zhao, Bo and Peng, Xiangyu and Zhu, Zheng and Yang, Shuo and Wang, Shuo and Huang, Guan and Bilen, Hakan and Wang, Xinchao and You, Yang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12196--12205},
  year={2022}
}
@article{dong2022privacy,
  title={Privacy for Free: How does Dataset Condensation Help Privacy?},
  author={Dong, Tian and Zhao, Bo and Lyu, Lingjuan},
  journal={arXiv preprint arXiv:2206.00240},
  year={2022}
}
